Domain Agnostic Few-Shot Learning For Document Intelligence

Few-shot learning aims to generalize to novel classes with only a few samples with class labels. Research in few-shot learning has borrowed techniques from transfer learning, metric learning, meta-learning, and Bayesian methods. These methods also aim to train models from limited training samples, and while encouraging performance has been achieved, they often fail to generalize to novel domains. Many of the existing meta-learning methods rely on training data for which the base classes are sampled from the same domain as the novel classes used for meta-testing. However, in many applications in the industry, such as document classification, collecting large samples of data for meta-learning is infeasible or impossible. While research in the field of the cross-domain few-shot learning exists, it is mostly limited to computer vision. To our knowledge, no work yet exists that examines the use of few-shot learning for classification of semi-structured documents (scans of paper documents) generated as part of a business workflow (forms, letters, bills, etc.). Here the domain shift is significant, going from natural images to the semi-structured documents of interest. In this work, we address the problem of few-shot document image classification under domain shift. We evaluate our work by extensive comparisons with existing methods. Experimental results demonstrate that the proposed method shows consistent improvements on the few-shot classification performance under domain shift.

==> main/deployment.tex <==
\section{Applications and Deployment}
Document image classification can find many enterprise level applications in insurance companies to reduce manual review and stream line claims processes. For example, casualty injuries claims usually have multiple correspondences with hospitals and clinics, each involving documents to be processed by the insurance company. Personal automobile claims processing can use automatic document classification of letters of guarantee, purchase receipts, and others in order to auto-approve a certain percentage of auto claim reimbursements. Each year, millions of claim related document images sent to insurance companies belonging to hundreds of categorizes related to financial institutions, medical providers, or legal organizations. A scalable document classifier can assign the correct categories as meta data to a document, which can be used to route to appropriate downstream tasks. Given the scale document image classification can be deployed in an enterprise, 
% an effective machine learning approach, 
an efficient framework for model training and iterations, together with an economical model hosting solutions has clear cost advantages.  
To support all those applications and achieve potential scalability , we are in the progress of deploying this trained model as an API under Container as a Service (CaaS) on AWS using Fargate managed Elastic Container Service (ECS). The efficient model size facilitates faster deployment and ease of maintenance. A standard ECS task with v4CPUs and 30G RAM can be used and the weights of the trained model can be conveniently packaged in a dockerized image and deployed at scale. 
% \textcolor{red}{but even large models can still be dockerized}









% 



==> main/methods.tex <==
\section{methods}
METHODS 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% DO NOT DELETE
    
% \begin{algorithm}[h!]
%  \caption{Efficent Graph Neural Network}
%     \begin{algorithmic}
%     \INPUT training documents $D = \{ (x_1, y_1), \dots (x_N, y_N) \}$.
%     \FOR {$m = 1, \dots, N$}
%         \STATE Extract text features with PyTesseract.
%         \STATE Detect document layout using PubLayNet.
%     \ENDFOR
%     \STATE Train word2vec on extracted text.
%     \STATE Convert output of PubLayNet into graph data.
%     \STATE Train GNN.
%     \OUTPUT Trained GNN network.
%         \end{algorithmic}
%         \label{psuedocode_copy}
%     \end{algorithm}
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
